Total Eclipse of the Heart -- Disrupting the InterPlanetary File System

Peer-to-peer networks are an attractive alternative to classical client-server architectures in several fields of application such as voice-over-IP telephony and file sharing. Recently, a new peer-to-peer solution called the InterPlanetary File System (IPFS) has attracted attention, which promises to re-decentralise the Web. Being increasingly used as a stand-alone application, IPFS has also emerged as the technical backbone of various other decentralised solutions and was even used to evade censorship. Decentralised applications serving millions of users rely on IPFS as one of their crucial building blocks. This popularity makes IPFS attractive for large-scale attacks. We have identified a conceptual issue in one of IPFS's core libraries and demonstrate their exploitation by means of a successful end-to-end attack. We evaluated this attack against the IPFS reference implementation on the public IPFS network, which is used by the average user to share and consume IPFS content. Results obtained from mounting this attack on live IPFS nodes show that arbitrary IPFS nodes can be eclipsed, i.e. isolated from the network, with moderate effort and limited resources. Compared to similar works, we show that our attack scales linearly even beyond current network sizes and can disrupt the entire public IPFS network with alarmingly low effort. The vulnerability set described in this paper has been assigned CVE-2020-10937. Responsible disclosure procedures are currently being carried out and have led to mitigations being deployed, with additional fixes to be rolled out in future releases.

==> eval-bootstrap2.tex <==
\section{Attacking a live IPFS 0.5 Bootstrap Node}
\label{appedix:bootsrap}
Shortly after the release of IPFS on April 28, 2020, Protocol Labs allowed us to evaluate our attack against one of the production bootstrap nodes from the default configuration that is shipped with IPFS.
This attack run was carried out over three hours in the live IPFS network in order to gauge the impact of the countermeasures deployed for IPFS 0.5.
The basic setting was equivalent to the evaluation performed using nodes operated specifically for evaluating our attack against the IPFS 0.5 countermeasures, as described in Section~\ref{sec:countermeasures}.
Figure~\ref{fig:xxx} illustrates the state of the bootstrap node's routing table over the course of a three-hour attack including some cool-down time.
Since this concrete attack run targeted a production system, the evaluation period was chosen such that results could be obtained to make and initial judgement regarding the deployed countermeasures utility without causing any real disruption to the network..
As can be seen, the results obtained from this run correlate with those presented in Figure~\ref{fig:default_rt_buckets_05}, illustrating that quick poisoning of a bootstrap node's routing table is not possible any more.
<<<<<<< HEAD
However, as long-running experiments have not yet been possible due to IPFS 0.5 being released on April 28, 2020, an accurate estimation of the costs for attacks against the network's bootstrap nodes is not yet available.
Long-running evaluations against IPFS 0.5 are underway to obtain such figures.
=======
However, after only one hour, the initial number of $ >200 $ honest peers in the bootstrap node's routing table could be more than halved and stayed below 100, clearly demonstrating the impact our attack still has on IPFS 0.5.
Still, since long-running experiments have not yet been possible due to IPFS 0.5 being released April 28, 2020, an accurate estimation of the costs for attacks against the network's bootstrap nodes is not yet available.
Long-running evaluations against IPFS 0.5 are underway to obtain such figures.
Protocol Labs's current position regarding attack difficulty compared to IPFS 0.4.23, is that fully poisoning a bootstrap node's routing table is still possible within several days at worst.
>>>>>>> 6b524cd53519f6c5941bc57931bdf27b343d06ba


==> rt_fig_counter_fixec_0_4.tex <==

\subfloat[Naive countermeasures for IPFS 0.4.23 to protect \gls{dht} peers from the ConnMgr's pruning routine.\label{fig:rt-04-counter}]{%
\begin{adjustbox}{height=0.4\textheight}

\includegraphics[width=\textwidth]{alex/ipfs-eclipse-figure4.pdf}




\end{adjustbox}
}



